Multi-frequency control and measurement of a spin-7/2 system encoded in a transmon qudit

Qudits hold great promise for efficient quantum computation and the simulation of high-dimensional quantum systems. Utilizing a local Hilbert space of dimension d > 2 is known to speed up certain quantum algorithms relative to their qubit counterparts given efficient local qudit control and measurement. However, the direct realization of high-dimensional rotations and projectors has proved challenging, with most experiments relying on decompositions of SU(d) operations into series of rotations between two-level subspaces of adjacent states and projective readout of a small number of states. Here we employ simultaneous multi-frequency drives to generate rotations and projections in an effective spin-7/2 system by mapping it onto the energy eigenstates of a superconducting circuit. We implement single-shot readout of the 8 states using a multi-tone dispersive readout (F_assignment = 88.3%) and exploit the strong nonlinearity in a high EJ/EC transmon to simultaneously address each transition and realize a spin displacement operator. By combining the displacement operator with a virtual SNAP gate, we realize arbitrary single-qudit unitary operations in O(d) physical pulses and extract spin displacement gate fidelities ranging from 0.997 to 0.989 for virtual spins of size j = 1 to j = 7/2. These native qudit operations could be combined with entangling operations to explore qudit-based error correction or simulations of lattice gauge theories with qudits. Our multi-frequency approach to qudit control and measurement can be readily extended to other physical platforms that realize a multi-level system coupled to a cavity and can become a building block for efficient qudit-based quantum computation and simulation.

==> 2024-03-28-oldabstract.tex <==
\begin{abstract}
\noindent Qudits hold great promise for efficient quantum computation and simulating high-dimensional quantum systems.
Utilizing a local Hilbert space of dimension $d > 2$ is known to speed up certain quantum algorithms relative to their qubit counterparts, enabled by gate sets providing universal control in $SU(d)$.
However, the direct realization of high-dimensional rotations and projectors has proved challenging, with most experiments relying on decompositions of $SU(d)$ operations into series of rotations between two-level subspaces of adjacent states and projective readout of a small number of states. 
Here we generate rotations and projections in an effective spin-$7/2$ system by mapping it onto the energy eigenstates of a superconducting circuit. 
We implement single-shot readout of the 8 states using a multi-tone dispersive readout ($F_{\rm assign} = 88 \%$) and exploit the strong nonlinearity in a high $E_J / E_C$ transmon to simultaneously address each transition and realize a spin displacement operator. 
By combining the displacement operator with a virtual SNAP gate, we realize arbitrary single-qudit unitary operations in at most $2(d - 1)$ physical pulses and extract spin-displacement gate fidelities ranging from $0.997$  to $0.989$ for virtual spins of size $j = 1$ to $j = 7 / 2$. 
These native local qudit operations could be combined with entangling operations to explore quantum error correction with spin-cat encodings or simulation of lattice gauge theories with qudits. As such, we expect that our demonstration of a highly controllable pseudo-spin can become a building block for efficient qudit based quantum computing and simulation. 
\end{abstract}
